TEEvil: Identity Lease via Trusted Execution Environments

We investigate identity lease, a new type of service in which users lease their identities to third parties by providing them with full or restricted access to their online accounts or credentials. We discuss how identity lease could be abused to subvert the digital society, facilitating the spread of fake news and subverting electronic voting by enabling the sale of votes. We show that the emergence of Trusted Execution Environments and anonymous cryptocurrencies, for the first time, allows the implementation of such a lease service while guaranteeing fairness, plausible deniability and anonymity, therefore shielding the users and account renters from prosecution. To show that such a service can be practically implemented, we build an example service that we call TEEvil leveraging Intel SGX and ZCash. Finally, we discuss defense mechanisms and challenges in the mitigation of identity lease services.

==> sections/old_stuff.tex <==
\section{ALL OLD STUFF BELOW THIS}


\section{Introduction}
Brief framing and selling points:
\begin{itemize}
    \item ``Automated'' crowdturfing makes it even easier for users to participate, and makes it desirable for both lessers and renters
    \item There are three main problems in spammy content generation:
    \begin{enumerate}
        \item Generate plausible content, that the spammer likes, and verifying it's been generated;
        \item Make it look like it is coming from real users;
        \item Be impactful.
    \end{enumerate}
    Using fake accounts can partially solve (1): content can be generated plausibly, and spammers are sure that it was published as it's under their control, but it cannot be personalized (as accounts are fake and do not have any contact with real users). However, many problems exist with (2) as fake accounts mantainers need to spend a lot of energies circumventing detection systems. Finally, regarding (3), impact is dubious.
    
    Using crowdturfing mechanisms solves (2): content comes directly from real user accounts (even if professional crowdturfers might have incentives to create fake accounts for the purpose). However, there are multiple problems with (1): content is created by the crowdturfer, and might be not what the paying spammer wants. Moreover, it is laborious and difficult to check that the content was really generated and posted, as it requires manual verification and needs to be accessible by the verifier. Again, impact is dubious: crowdturfing tasks are usually performed on ``open'' opinion websites, where little pre-established trust exists, therefore there is little extra impact of a real account with respect to fake accounts.
    
    Using influencers solves nicely (1) and (2), but regarding (3) they suffer from problems of scale: reach and impact could be amplified by e-word-of-mouth marketing. 
    
    Another problem of crowdturfing: can be detected by ML, however, detection can be evaded by playing the right game~\cite{wang2014man}, it would be easier to avoid detection from the enclave
    
    We present a new turfing technique that \textbf{solves efficiently all three issues}: content is generated by the spammer/renter, can be personalized according to the writing style of the rented accounts. Posting on behalf of the renter is automatically verified (solving verification issues), and is proxied through real user accounts. Finally, as content is posted on real user accounts, for their friends to see, it maximizes impact as we leverage pre-existing trust relationship between people, as renters pose to be the real users generating content or interactions.
    \item Similar reasoning applies when buying interactions (e.g., ``like'' interactions on social networks).
\end{itemize}

\noindent List of motivating things:
\begin{itemize}
    \item QAnon case: from 4chan some guys created the hoax of pedophilia and satanic rituals involving Democrat politicians in the USA, then moved to Reddit where they got visibility through some good initial visibility. Now at every Trump rally you can see people with QAnon flags and T-shirts.
    \item Brazilian elections: WhatsApp groups to spread fake news pro one candidate -- would be even more effective if the group was created by your friend
    \item For recommenders: the case of ElsaGate on YouTube, how all these videos were recommended immediately after kids' videos.
    \item Appear trustworthy using reputation: sites like TripAdvisor are full of bought reviews. This is why we trust reputable accounts: people with years of history of interaction in the community, and hundreds of posts.
    \item Appear trustworthy using pre-existing trust: if my friends post about something, I might be inclined to trust them.
    \item Watering down political statements: similar to the previous point. If I know that my friend and I have similar political opinions, and then one day he expresses not-negative views about something opposed to our opinions (e.g., ``maybe he has a point'' referred to Trump, if we suppose that my friend is a Democrat).
    \item An ``automatic'' extension to the previous point: that's how implicitly recommender systems work -- by suggesting to users what like-minded people liked. If we can have like-minded people to like something, we can pollute the recommender.
    \item E-voting is a simple yet very impact full process for any democracy and it provides a very simple use-case for \name{}. 
\end{itemize}

\noindent What such a platform enables:
\begin{itemize}
    \item A new distributed advertising paradigm: companies pay people to influence their peers, rather than paying a platform to passively show ads to people;
    \item Disruption of trust between people, as you can't know if your friends or a company is writing/doing something;
    \item Quick buildup of plausible/realistic ``consensus'', to bootstrap content virality or exaggerate support to some cause.
\end{itemize}


\section{Building Blocks}
Here we list the building blocks of our turfing technique and whether there already exists relevant literature about it.
\begin{enumerate}
\item Renter asks the platform to rent accounts to perform some action X on social networks for Y cryptomoneys. This action X can be as simple as a ``like'' or ``reshare'', up to complex interaction, e.g., comments, posts, reviews.
\item The platform now needs to select a subset of all enrolled accounts to offer to the renter. This needs to take into account the maximum budget, but also the renter goals. his depends on the type of desired activity, and leads to different strategies:
    \begin{itemize}
        \item To maximize exposure of some content (influencer friends / advertisement) through posting, or liking or resharing, in order for social friends to see the content. This problem is called influence maximization~\cite{kempe2003maximizing}, and interestingly can be done topic-wise~\cite{Barbieri2012,Chen2015,Goyal2011} in order to closely emulate current OSNs advertising capabilities.
        \item To ``water down'' or ``sneak in'' some opposite views on echo chambers of strong supporters of some polarized topic~\cite{del2016echo,del2016spreading}, as cross-opinion sharing is usually unlikely for a number of reasons (tendency to aggregate with like-minded users, confirmation biases, and algorithmically determined exposure to news that is influenced by what our friends like, in Facebook~\cite{bakshy2015exposure}). Here you want to pick influential users on given echo chambers. Another possibility is to initiate conflicts with ``opposing'' communities, and these types of conflicts are usually initiated by a few influencial users, but then carried out by less active community members~\cite{kumar2018community} -- suggesting that only initial bootstrap would be needed.
        \item To quickly build up consensus in some community, strategies might be to select active users of such communities, or just a high quantity of cheap accounts that can sustain a constant flow of interactions.
        \item To bootstrap virality, maximizing exposure, and knowledge of different ranking algorithms for different social networks (e.g., the imgur OSN ranks content as viral if it exceeds a threshold of ``likes'' within a given interval of time) might do the trick. Here there exist some works that show precise patterns of content virality~\cite{dow2013anatomy,cheng2014can,friggeri2014rumor}, that can be leveraged both in selection of accounts (here, probably the important part is more in the ``timing'' of interaction, so many cheap accounts might work, as long as they are ``spread out'' in the network). When virality is bootstrapped and content has visibility, it will continue spreading autonomously: it was observed that bots do not accelerate (fake) news diffusion, as people are prone to sharing such content~\cite{Vosoughi1146}. Moreover, key value for virality is overcoming natural ``user passivity''~\cite{romero2011influence} -- we realize this thanks to the rental scheme, that could be then better than conventional ``few famous influencer'' virality techniques.
        \item It was shown that different nodes (e.g., normal people vs popular influencers) contribute differently to different types of content diffusion, such as simple sharing versus engaging with friends, or even do something in the real world~\cite{cheng2018diffusion}.
    \end{itemize}
    Ultimately, according to the maximizing strategy, the platform needs to give a monetary value to accounts (or to estimate what kind of diffusion could be obtained with that amount of money), and to pick a set of potential lessors.
\item The platform asks selected potential lessors, through some app, whether they are interested in allowing to perform the requested action on their OSN account for a given amount of money.
\item Account of users that consent is now rented to the renter to perform the specified action. Control switches to an SGX enclave running a system such as DelegaTEE, programmed to perform the specific action on the specified target. Our platform ensures that the TEE enclave only does what was agreed -- however, the lessor can also attest to the remote enclave to make sure of what is being executed.
\item The enclave generates the required content, if needed, and then submits it on the social network; or performs the required interaction. This is performed through a proxy app on the lessor's phone, to bypass OSN anomaly detection algorithms.
There are a number of details to consider, depending on the type of action:
\begin{itemize}
    \item For \textbf{content to generate}, such as posts and comments, there are many techniques that can be used to generate realistic text variants (such as fake reviews)~\cite{yao2017automated,juuti2018stay}. \todo{continue}
    \item Performing any type of action (including, e.g., reshares, ``likes'') needs to take into account anomaly detection mechanisms of the online platforms, e.g., time and geographical origin of the action, plausible browsing patterns. We bypass geolocation attempts by requiring that interactions come from users' smartphones, thanks to a proxy application. Time and browsing patterns can be modeled instead, according to average behaviors of users in online platforms~\cite{benevenuto2009characterizing}.
\end{itemize}


Potential mining of lessor's previous writing style (or similar customizations), to ensure personalized actions, should be done by the enclave. 

\item how to generate plausible interactions:
    \begin{itemize}
        \item actions (like share etc)
        \item text
    \end{itemize}
\item When to do interaction
    \begin{itemize}
        \item need to bypass outliar checks?
        \item patterns to make stuff go viral
    \end{itemize}
\item how to bypass content censorship: as long as it's not character
\item Related to social media posting: compared to existing crowdturfing we don't need to verify the submission of a user because it's done automatically
\item We need to check if there exist a website that allows crowdturfing and already allows payments through a cryptocurrency 
\end{enumerate}

\section{Unresolved/Open Issues}
\begin{enumerate}
    \item A platform that wants to stop our technique might as well start renting accounts, making them post some unique content (or interact with something specific), then search for it in their platform, thus deanonimizing users of the service. Then, it could suspend/warn the offending accounts.
    \begin{itemize}
        \item One counterargument is that OSNs could already do this (e.g., go to websites, buy fake followers, point them to an account of them, then ban them all), but they don't. Plus, there would not be so much research effort in sybil/bot detection.
        \item Another argument could be that our turfing technique could require for some ``anonimity'' to be in place, in case of interactions (e.g., already existing and incoming ``likes''). The problem still holds for content creation.
        \item A third argument could be to make it economically unfeasible for OSNs -- but this is still open discussion.
    \end{itemize}
\end{enumerate}


==> sections/threatmodel.tex <==
\section{Threat Model}
\label{sec:threat_model}


We consider an attacker interested in stopping \name{}. To achieve this goal the attacker is after at least one of the following objectives: (i) removing the incentives to participate in the protocol for account owners, account renters, or both; (ii) exposing users of \name by compromising the privacy of the system. For now, we exclude denial of service (DoS) attacks from the threat model, and discuss about possible DoS mitigations in Section~\ref{sec:discussion}.


\paragraph{Removing Incentives.} While incentives are different for the various entities of the protocol, they are intrinsically linked. \Users are offering a service by renting their accounts, and if they are not compensated for providing this service they will not have any incentive to participate in \name{}. \Requesters seek to maximize the effectiveness of their campaign; they rely on \name{} to reach their goals while avoiding being linked to the campaign in the process. Therefore, the absence of a good base of \users will deter \requesters from promoting campaigns in \name{}, as other well-established platforms would be more impactful. Consequently, if an attacker can prevent payments to a significant amount of \users, it can start a chain reaction in which \users withdraw from \name{}, causing \requesters to discontinue or not launch any new campaign, thus pushing even more users to leave, and so on. In summary, this is equivalent to breaking the \emph{fairness} property.

\paragraph{Exposing Users.} This is equivalent to breaking the \emph{indistinguishability} or \emph{plausible deniability} properties, and has similar consequences to removing incentives: users leaving \name. User involvement in \name would often violate ToS, or infringe the law. Exposure will push \users out of \name, thus creating the same chain reaction described when removing incentives. The impact of exposure on account renters exacerbates the problem even more. For example, if someone can prove a link between a renter and a specific campaign, the illusion of grass-root support and thus one of the advantages of \name would be gone.



\subsection{Attacker Model}

\paragraph{Enclave Adversaries.}
We assume the standard SGX adversary model against \name enclaves. In particular, the \enclinf controls the OS in which the enclaves run (i.e., has privileged code execution), and can tap into the memory bus, but cannot tamper with the CPU package. Additionally, the \enclinf can delay or drop any network packet from and to the enclave -- however, can not see the content of packets if the enclave serves as the TLS endpoint.
We assume no adversary can compromise the enclaves -- this means that we rely on the security properties provided by SGX and the underlying cryptographic mechanisms. We trust the TEE manufacturer (i.e., Intel) to not fake attestation queries, or otherwise compromise the security of any SGX capable CPUs, either voluntarily or under coercion from an external party. Rollback attacks are out of scope -- we refer the interested reader to~\cite{matetic2017rote,brandenburger2017rollback}.



\paragraph{Protocol Participants Adversaries.}
The \user, \requester, and \enclinf have full control over their devices, and they could be byzantine. We don't provide any guarantee for the byzantine party (e.g., we cannot stop them from exposing themselves as part of \name) -- in this case, the remaining ``honest'' parties should still benefit from all the security properties described in Section~\ref{sec:prob_statement}.
Any participant in the protocol of \name, and any third party, can pose as adversary. We assume the adversary can gain unprivileged access to any device of other protocol participants, and can manipulate local Internet traffic around  protocol participants, e.g., eclipsing their view of the cryptocurrency blockchain. However, the adversary does not control the whole point-to-point Internet traffic between protocol participants and target services.
We observe that privileged code execution on the device of \users or \requesters by an adversary is equivalent to the case in which the user is byzantine -- properties provided by \name cannot be guaranteed to the compromised entity.

\Users, \requesters, and \enclinfs can collude with each other in order to gain an advantage to the non-colluding party, or to violate security properties of \name. However, services targeted by \name can \textbf{not} collude with any other protocol participant: we discuss the implications of such a powerful adversary in Section~\ref{sec:discussion}.

